Consistency Deep Equilibrium Models

Deep Equilibrium Models (DEQs) have emerged as a powerful paradigm in deep learning, offering the ability to model infinite-depth networks with constant memory usage. However, DEQs incur significant inference latency due to the iterative nature of fixed-point solvers. In this work, we introduce the Consistency Deep Equilibrium Model (C-DEQ), a novel framework that leverages consistency distillation to accelerate DEQ inference. We cast the DEQ iterative inference process as evolution along a fixed ODE trajectory toward the equilibrium. Along this trajectory, we train C-DEQs to consistently map intermediate states directly to the fixed point, enabling few-step inference while preserving the performance of the teacher DEQ. At the same time, it facilitates multi-step evaluation to flexibly trade computation for performance gains. Extensive experiments across various domain tasks demonstrate that C-DEQs achieve consistent 2-20$\times$ accuracy improvements over implicit DEQs under the same few-step inference budget. Our code is available at https://github.com/landrarwolf/CDEQ.

==> inputs/tables/wikitext_others.tex <==
\begin{tabular}{lccc}
\toprule
\textbf{Model} & \textbf{\# Params} & \textbf{NFE} & \textbf{Memory (GB)} \\ \midrule

Generic TCN~\cite{bai2018empirical} & 150M & - & - \\
GCNN~\cite{dauphin2017language} & 230M & -& - \\
AWD-QRNN~\cite{merity2018analysis} & 159M & - & 7.1 \\
Transformer-XL~\cite{dai2019transformer} & 165M & - & 8.5 \\
\midrule

DEQ~\cite{bai2019deq} & 171M & 1 & 3.1\\
NDEQ~\cite{bai2021ndeq} & 173M & 1 & 3.1\\
\textbf{C-DEQ (Ours)} & 173M & 1 & 3.2\\ \midrule

DEQ~\cite{bai2019deq} & 171M & 10 & 3.2\\
NDEQ~\cite{bai2021ndeq} & 173M & 10 & 3.3\\
\textbf{C-DEQ (Ours)} & 173M & 10 & 3.3\\ \midrule

DEQ~\cite{bai2019deq} & 171M & 20 & 3.3\\
NDEQ~\cite{bai2021ndeq} & 173M & 20 & 3.3\\
\textbf{C-DEQ (Ours)} & 173M & 20 & 3.3\\ \midrule

DEQ~\cite{bai2019deq} & 171M & 30 & 3.3\\
NDEQ~\cite{bai2021ndeq} & 173M & 30 & 3.4\\
\textbf{C-DEQ (Ours)} & 173M & 30 & 3.4\\ \midrule

DEQ~\cite{bai2019deq} & 171M & 40 & 3.4 \\
NDEQ~\cite{bai2021ndeq} & 173M & 40 & 3.4\\ 
\textbf{C-DEQ (Ours)} & 173M & 40 & 3.4\\
\bottomrule
\end{tabular}

